Assessing and Improving the Mutation Testing Practice of PIT

Mutation testing is used extensively to support the experimentation of software engineering studies. Its application to real-world projects is possible thanks to modern tools that automate the whole mutation analysis process. However, popular mutation testing tools use a restrictive set of mutants which do not conform to the community standards as supported by the mutation testing literature. This can be problematic since the effectiveness of mutation depends on its mutants. We therefore examine how effective are the mutants of a popular mutation testing tool, named PIT, compared to comprehensive ones, as drawn from the literature and personal experience. We show that comprehensive mutants are harder to kill and encode faults not captured by the mutants of PIT for a range of 11% to 62% of the Java classes of the considered projects.

==> discussion.tex <==

This section discusses our findings, in Section \ref{sec:Findings}, %implications, in section \ref{sec:Implications}, 
and threats to validity of the present study, in Section \ref{sec:Threats}. 

%These are categorized as usual, i.e.,  according to "Construct Validity" \ref{sec:constrval}, Internal Validity, \ref{sec:internval}, and External Validity, \ref{sec:externval}.


\subsection{Findings}\label{sec:Findings}
%-Disjoint mutants numbers
%\subsection{Implications}\label{sec:Implications}

The most important finding of our study is that mutation testing tools should use the comprehensive mutant set instead of the popular one. For instance, it is important to include all the instances of relational and arithmetic mutants, as suggested by the literature \cite{AndrewsBLN06, OffuttH96}. Regarding PIT, despite the attempts made in its previous updates included in its latest version, it still has several weaknesses, as our study show. To fulfil this need, we augmented the tool with the comprehensive mutants and plan to submit them for inclusion in its future releases. 

Another issue arises from the use of disjoint mutants. As demonstrated by our results, there is a large variation when considering all the mutants instead of the disjoint ones. Though, from both figures \ref{objectivecomp} and \ref{easiness}, it becomes evident, from the differences between the two measurements, that there is an inflation effect on the measurement of all mutants, i.e., the volume of the dark coloured area is much smaller. Therefore, future research should also report the disjoint mutants measurements. %This involves some additional cost, however, it is practically feasible as our results show. 

Our results also suggest that there is a second parameter that can inflate the used measurements. This is the difference between the examined project classes. As it can be seen in Table \ref{operators_table}, there is a large variation on the number of mutants per class, from none to thousands, and the mutation score varies from zero to one. Since mutation testing applies to unit testing, treating a project as a whole results in inflating the measurements and leaves program parts untested. This is clearly visible in Figure \ref{objectivecomp}. Since the goal of mutation testing is to thoroughly test every part of the code under investigation to establish confidence on its function, it is mandatory to reduce the inflation effects of the employed measurements.

Another way to see this last point is to consider mutants' easiness. Clearly, it does not make sense to compare strategies with mutants of easiness 1, i.e., killed by all the test cases that exercise them. In such cases, mutants are equivalent to statement coverage. As it is shown in Figure \ref{easiness}, more than half of all the studied classes contain trivial mutants. Disjoint mutants suffer less from this effect, but still their consideration can influence the reported results. 


Mutants' easiness provides additional explanations on our results. By considering classes with non-trivial mutants, i.e., with an easiness lower than 1, we observe large differences between the examined mutants. Thus, the comprehensive mutants are harder to kill than the common ones in nearly all the cases. This is reflected in both adopted measurements, demonstrating the practical significance of our results. 

%Finally, based on our results we should 
%However, disjoint mutants clearly reflect the differences between the examined approaches and thus, 


%The comprehensive mutant set can be seen as an attempt to close the wholes in the implementation of PIT. We provide evidence that these are important and should be closed.  


\subsection{Threats to Validity}\label{sec:Threats}

\subsubsection{Construct Validity}\label{sec:constrval}

Threats to construct validity can arise when considering  measures that do not represent the actual intended ones. With respect to the mutation score and the disjoint mutants measurements, we intend to measure the ability of the employed test cases to thoroughly exercise all parts of the code under test. Previous research \cite{Offutt11, offutt1996subsumption} has shown this practice to be valid. Moreover, our evaluation is in line with previously reported results, thus, reducing this risk. 

Previous research has also established a link between mutation score and actual fault detection \cite{AndrewsBL05, AndrewsBLN06}. Thus, the comprehensive mutant set is based on these studies. Additionally, the comprehensive set is a superset of the commonly used one and thus, it can indicate potential weaknesses of the common mutants. This is shown with both the difficulty and score measurements, which are common in mutation literature. Finally, it is important to mention that the employed subjects are mature and widely used by actual practitioners and researchers. Therefore, using their test suites should be appropriate. Future research will deepen our understanding of what is an adequate test suite. 

\subsubsection{Internal Validity}\label{sec:internval}

Threats to internal validity arise when considering potential issues with the conclusions coming from the observed measurements. We use non-adequate
test suites since this is the current practice \cite{GligoricGZSAM15} and the determination of infeasible test requirements is practically infeasible.
Additionally, the comprehensive mutants clearly tend to be harder to kill than the common ones and thus having the potential to lead to stronger tests \cite{JiaH09a}. Nevertheless, it is noted that at the time of the experiment, we did not know which mutants should be used. These were determined based on literature and the authors' experience. It is noted that there were relevant discussions during the 2014 and 2015 mutation testing workshops concluding that the comprehensive mutants should be of actual use.

Other issues can be due to the use of PIT and the enhancements we made.  These could contain errors that potentially affect our results. However, we carefully checked our implementations and compared with the current ``out of the box'' version of PIT.  %and performed a mutant quality evaluation. 
Since PIT is widely used, possible implementation bugs should not be severe. 

It is important to note that PIT operates on Java bytecode. To this end, PIT first gathers coverage information about the test suite that is given and check if the suite is ”green”, i.e., it checks that all the tests pass on the original (unmutated) code and then, mutates the program using the selected operators. This practice may result in lower quality when comparing with mutation applied on source code. However, previous research with bytecode tools performing branch coverage suggests that bytecode analysis is valid and in many cases underestimates the actual measurements when compared with the source code \cite{LiMOD13}. Similarly, bytecode mutation looses the information of the logical operators and thus, there might be issues with the absence of these mutants. However, these mutants should be covered by the relational and conditional operators. Indeed, these mutants should result in clause coverage \cite{LiMOD13} and since the requirement is to strongly kill them, they should probably subsume the logical ones, unless they are equivalent .

To reduce all the above-mentioned threats, we will also make all of our data and the extended version of PIT publicly available\footnote{If, and when the paper is accepted.}.% to further reduce the mentioned threat.



\subsubsection{External Validity}\label{sec:externval}

Threats to external validity arise when considering possible issues with the generalization of the reported results. In the present study, we used 5 real-world projects, from different application domains, and different sizes. Most of them have been used in recent studies with the same settings. Since, our results are consistent across the selected programs and are in line with the beliefs of the community \cite{MutKeynote2015} we believe that this threat is limited. Still, there are many factors, e.g., test suites, programs and tools, that can affect the generalization of our findings. Though, our goal was to show potential weaknesses of previous studies under similar settings. 


==> threats.tex <==
This section discusses the limitations and threats to validity of the present study. These are categorized as usual, i.e.,  according to "Construct Validity" \ref{sec:constrval}, Internal Validity, \ref{sec:internval}, and External Validity, \ref{sec:externval}.


\subsection{Construct Validity}\label{sec:constrval}

Threats to construct validity can arise when considering  measures that do not represent the actual intended ones. With respect to the mutation score and the disjoint mutants measurements, we intend to measure the ability of the employed test cases to test thoroughly all parts of the code under test. Previous research \cite{Offutt11, offutt1996subsumption} has shown this practice to be valid. Moreover, our mutant quality evaluation is in line with previously reported results, thus, reducing this risk. 

Previous research has also established a link between mutation score and actual fault detection \cite{AndrewsBL05, AndrewsBLN06}. Though, the comprehensive mutant set is based on these studies. Additionally, the comprehensive set is a superset of the commonly used one and thus, it can indicate potential weaknesses of the common mutants. This is shown with both the difficulty and score measurements, which are common in mutation literature. Finally, it is important to mention that the employed subjects are mature and widely used by actual users and researchers therefore, using their test suites should be appropriate. Future research will deepen our understanding of what is an adequate test suite. 

\subsection{Internal Validity}\label{sec:internval}

Threats to internal validity arise when considering potential issues with the conclusions coming from the observed measurements. We use non-adequate
test suites since this is the current practice \cite{GligoricGZSAM15} and the determination of infeasible test requirements is practically infeasible. Additionally, at the time of the experiment, we did not know which mutants should be used. These were determined based on the authors' experience and the discussions made during the 2014 and 2015 mutation testing workshops.

Other issues can be due to the use of PIT and the enhancement we made.  These, could contain errors that potentially affect our results. However, we carefully check our implementations and performed a mutant quality evaluation. Also, PIT is widely used and thus, bugs related to test execution and evaluation should not be severe. 

It is important to note that PIT operates on Java bytecode. To this end, PIT first gathers coverage information about the test suite that is given and check if the suite is ”green”, i.e., it is checked that all the tests pass on the original (unmutated code) and then, mutates the program using the selected operators. This practice may result in problems when comparing with mutation applied on source code. However, previous research with bytecode tools performing branch coverage suggests that bytecode analysis is valid and in many cases underestimates the actual measurements when compared with the source code \cite{LiMOD13}. Similarly, bytecode mutation looses the information of the logical operators and thus, there might be issues with the absence of these mutants. However, these mutants should be covered by the relational and conditional operators. Indeed, these mutants should result in clause coverage \cite{LiMOD13} and since the requirement is to strongly kill them, they should prod-subsume the logical ones, unless they are equivalent .

To reduce all the above-mentioned threats, we will also make all of our data and the extended version of PIT publicly available\footnote{If, and when the paper is accepted.} to further reduce the mentioned threat.



\subsection{External Validity}\label{sec:externval}

Threats to external validity arises when considering possible issues with the generalization of the reported results. In the present study, we used 5 real-world projects, from different application domains, and different sizes. Most of them have been used in resent studies with the same settings. Since, our results are consistent across the selected programs and are in line with the beliefs of the community \cite{MutKeynote2015} we believe that this threat is limited. Still, there are many factors, e.g., test suites, programs and tools, that can affect the generalization of our findings. Though, our goal was to show potential weaknesses of previous studies under similar settings.
